Flat Metric Minimization with Applications in Generative Modeling

We take the novel perspective to view data not as a probability distribution but rather as a current. Primarily studied in the field of geometric measure theory, $k$-currents are continuous linear functionals acting on compactly supported smooth differential forms and can be understood as a generalized notion of oriented $k$-dimensional manifold. By moving from distributions (which are $0$-currents) to $k$-currents, we can explicitly orient the data by attaching a $k$-dimensional tangent plane to each sample point. Based on the flat metric which is a fundamental distance between currents, we derive FlatGAN, a formulation in the spirit of generative adversarial networks but generalized to $k$-currents. In our theoretical contribution we prove that the flat metric between a parametrized current and a reference current is Lipschitz continuous in the parameters. In experiments, we show that the proposed shift to $k>0$ leads to interpretable and disentangled latent representations which behave equivariantly to the specified oriented tangent planes.

==> macros.tex <==
%\usepackage{pgfplots}
%\pgfplotsset{compat=newest}
%% the following commands are sometimes needed
%\usetikzlibrary{plotmarks}
%\usepackage{grffile}

%\usepackage{latexsym}
\usepackage[english]{babel}
% %\usepackage{rotating}
\usepackage{subfig}
%\usepackage{multibbl}
%\usepackage{calc}
%\usepackage{lastpage}
\usepackage{amsmath,epsfig,amssymb,amsbsy, amsthm, mathabx}
%\usepackage{euproposal}
%\usepackage{multirow}
%\usepackage{natbib}
%\usepackage{multibib}
%\usepackage{fancybox}
%\usepackage{nicefrac}
%\usepackage[table]{xcolor}
%\usepackage[right]{eurosym}
%\usepackage{bbm}


%\usepackage[bordercolor=white,backgroundcolor=gray!30,linecolor=black,colorinlistoftodos]{todonotes}

%\usepackage[T1]{fontenc}

%\usepackage{wrapfig,graphicx}
%\usepackage{url}
%\usepackage{titlesec}

%\usepackage{color}
%\usepackage{colortbl}


%\newcommand{\jl}[1]{\todobase{J}{#1}{yellow}}
\newcommand{\cThomas}[1]{ {\color{blue} #1 }}
%\newcommand{\mm}[1]{\todobase{J}{#1}{cyan}}

\newcommand\dimOmega{d}
\newcommand{\ngradients}{m}
\newcommand{\mfindex}{k} %k
\newcommand{\unarycost}{s}
\newcommand{\mfweights}{b}
\newcommand{\bitem}{\begin{itemize}}
\newcommand{\eitem}{\end{itemize}}
\newcommand{\mc}[1]{\mathcal{#1}}
\newcommand{\mb}[1]{\mathbb{#1}}
\newcommand{\R}{\mathbf{R}}
\newcommand{\B}{\mathbb{B}}
\newcommand{\U}{\mathbb{U}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\PP}{\mathbb{P}}
\newcommand{\bpm}{\begin{pmatrix}}      
\newcommand{\epm}{\end{pmatrix}}
\newcommand{\T}{\top}
\newcommand{\tr}{\mathsf{tr}}
\newcommand{\ol}[1]{\overline{#1}}      
\newcommand{\la}{\langle}
\newcommand{\ra}{\rangle}
\newcommand{\si}{\sigma}
\newcommand{\mrm}[1]{\mathrm{#1}}
\newcommand{\msf}[1]{\mathsf{#1}}
\newcommand{\Diag}{\mathrsf{Diag}}
\newcommand{\row}[2]{{#1}_{#2,\bullet}}
\newcommand{\col}[2]{{#1}_{\bullet,#2}}
\newcommand{\veps}{\varepsilon}
\newcommand{\toset}{\rightrightarrows}
\newcommand{\w}{\omega}
\newcommand{\gdw}{\Leftrightarrow}
\newcommand{\vphi}{\varphi}
\newcommand{\tmop}[1]{\ensuremath{\operatorname{#1}}}
\newcommand{\norm}[1]{\Vert #1 \Vert}
\newcommand{\normc}[1]{| #1 |}
\newcommand{\bbR}{\mathbb{R}}
\newcommand{\bbZ}{\mathbb{Z}}
\newcommand{\bbRext}{\mathbb{R} \cup \{ \infty \} }
\newcommand{\bbN}{\mathbb{N}}
\providecommand{\iprod}[2]{\langle#1,#2\rangle}


\newcommand{\bi}{\begin{itemize}}
\newcommand{\ei}{\end{itemize}}
\newcommand{\HH}{\mathcal{H}}
\newcommand{\MM}{\mathcal{M}}

\newcommand{\DD}{\mathcal{D}}
\newcommand{\JJ}{\mathcal{J}}
\newcommand{\Ss}{\mathcal{S}}

\newcommand{\reps}{\rho_{\veps}}
\newcommand{\geqs}{\geqslant}
\newcommand{\leqs}{\leqslant}


%\newcommand{\cref}[1]{ [{#1}]}
\newcommand{\cref}[1]{ {\tiny[{#1}]}}
%\newcommand{\tm}[1]{[#1] }
\newcommand{\tm}[1]{}

\newcommand{\VI}{\mathsf{VI}}
\newcommand{\SOL}{\mathsf{SOL}}
\newcommand{\graph}{\mathsf{gph}}
\newcommand{\conv}{\mathsf{conv}}
\newcommand{\rint}{\mathsf{rint}}
\newcommand{\bd}{\mathsf{bd}}
\newcommand{\rge}{\mathsf{rge}}
\newcommand{\epi}{\mathsf{epi}}
\newcommand{\lev}{\mathsf{lev}}
%\newcommand{\argmin}{\mathsf{argmin}}
%\newcommand{\argmax}{\mathsf{argmax}}

\newcommand{\detail}{\ding{43} \structure{Detail}}

\newcommand{\fr}[3][]{\frame{\frametitle{#2}\begin{textblock*}{6cm}(12cm,1.5cm)\rotatebox{90}{\parbox{7cm}{\scriptsize\structure{#1}}}\end{textblock*}\bi #3 \ei}}
\newcommand{\frb}[3][]{\frame{\frametitle{#2}\begin{textblock*}{6cm}(12cm,1.5cm)\rotatebox{90}{\parbox{7cm}{\scriptsize\structure{#1}}}\end{textblock*}#3}}
\newcommand{\tmemtitle}{\textbf}

%\newcommand{\mathbbm}{\mathbb}
\newcommand{\C}{\mathcal{C}}
\newcommand{\D}{\mathcal{D}}
\newcommand{\Rn}{\mathbb{R}^n}
\newcommand{\Rm}{\mathbb{R}^m}
\newcommand{\Rmxn}{\mathbb{R}^{m \times n}}
\newcommand{\Rd}{\mathbb{R}^d}
\newcommand{\Rl}{\mathbb{R}^L}
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\beqa}{\begin{eqnarray}}
\newcommand{\eeqa}{\end{eqnarray}}
\newcommand{\bc}{\begin{center}}
\newcommand{\ec}{\end{center}}
\newcommand{\lcb}{\left\{}
\newcommand{\rcb}{\right\}}
\newcommand{\lbr}{\left(}
\newcommand{\rbr}{\right)}
\newcommand{\seq}{\subseteq}
\newcommand{\PC}{\Pi_{\C}}
\newcommand{\PD}{\Pi_{\D}}
\newcommand{\assign}{:=}
\newcommand{\Om}{\Omega}
\newcommand{\BV}{\tmop{BV}}
\newcommand{\SBV}{\tmop{SBV}}
\newcommand{\Ccinf}{C_c^{\infty}}
\newcommand{\Dloc}{\D_{\tmop{loc}}}
\newcommand{\Hausd}{\mathcal{H}}
\newcommand{\tmtextbf}[1]{{\bfseries{#1}}}
\newcommand{\tmtextit}[1]{{\itshape{#1}}}
\newcommand{\tmem}[1]{{\em #1\/}}
%\newcommand{\subs}[1]{\smallskip\noindent\textbf{#1.} }
\newcommand{\subs}[1]{\medskip\noindent\textbf{#1.} }
%\newcommand{\subs}[1]{\noindent\textbf{#1.} }
%\newcommand{\subs}[1]{\paragraph{#1.} }

\newcommand{\wi}{.1\columnwidth}

\newcommand \M   {{\mathcal{M}}}                     % manifold

\newcommand \Sone       {{{\Ss}^1}}                           % S^1
\newcommand \TVS        {{TV_\Sone}}                        % TV_{S^1}
\newcommand \TVM        {{TV_\M}}                        % TV_{S^1}
\newcommand \Stwo       {{{\Ss}^2}}                           % S^1
\newcommand \TVStwo        {{TV_\Stwo}}                        % TV_{S^1}
\newcommand \TVSg       {{TV_\Sone^g}}                      % TV_{S^1}^g
\newcommand \TV         {{TV}}                              % TV
\newcommand{\dx}         {\,dx}
\newcommand \Su         {{S_u}}                             % subset
% of Omega w 
\newcommand \omegaDim   {{m}}                               % image domain dimension
\newcommand \dH         {{d\;\!\mathcal{H}^{\omegaDim-1}}}  % Hausdorff measure
\newcommand{\Div}{\tmop{Div}}


%\arrayrulecolor{black} % green tables otherwise
%\renewcommand{\familydefault}{\sfdefault}
%\usepackage{arial}

\newcommand{\fc}{^{\ast}}
\newcommand{\fcc}{^{\ast\ast}}
\newcommand{\ow}{\text{otherwise}}

\newcommand{\RL}{\R^L}
\newcommand{\Rb}{\bar{\R}}

%\newtheorem{thm}{Theorem}[section]
%\newtheorem{prop}[thm]{Proposition}

\newtheorem{thm}{Theorem}
\newtheorem{defi}{Definition}
\newtheorem{lem}{Lemma}
\newtheorem{prop}{Proposition}
\newtheorem{cor}{Corollary}
\newtheorem{rem}{Remark}
\newtheorem{conj}{Conjecture}
\newtheorem{ex}{Example}
\newtheorem{clm}{Claim}

\newcommand{\dat}{\boldsymbol{\rho}}
\newcommand{\dats}{\boldsymbol{\sigma}}
\newcommand{\reg}{\boldsymbol{\Phi}}
%\newcommand{\Gr}{\mathbf{1}}
\newcommand{\ul}{\boldsymbol{u}}
\newcommand{\el}{\boldsymbol{e}}
\newcommand{\vl}{\boldsymbol{v}}
\newcommand{\Vl}{\boldsymbol{V}}
\newcommand{\gl}{\boldsymbol{g}}
\newcommand{\pl}{\boldsymbol{p}}
\newcommand{\ql}{\boldsymbol{q}}
\newcommand{\nl}{\boldsymbol{q}}
\newcommand*\Bell{\ensuremath{\boldsymbol\ell}}
\newcommand*\Bgamma{\ensuremath{\boldsymbol\gamma}}

\newcommand{\one}[1]{\mathbbm{1}_{#1}}

\newcommand*{\vertbar}{\rule[-1ex]{0.5pt}{2.5ex}}

\newcommand{\measurerestr}{%
  \,\raisebox{-.127ex}{\reflectbox{\rotatebox[origin=br]{-90}{$\lnot$}}}\,%
}

%\newcommand{\epi}{\operatorname{epi}}
\newcommand{\id}{\mathsf{id}}

\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\LM}{\mathbf{\Lambda}}

\DeclareMathOperator{\KL}{KL}
\DeclareMathOperator{\argmin}{arg\,min}
\newcommand{\Lip}{\text{Lip}}
\newcommand{\im}{\text{im}}
\newcommand{\prox}{\text{prox}}
\newcommand{\dom}{\text{dom}}
\newcommand{\tow}{\mathrel{\ensurestackMath{\stackon[1pt]{\rightharpoonup}{\scriptstyle\ast}}}}

\newcommand{\bbM}{\mathbb{M}}
\newcommand{\bbF}{\mathbb{F}}
\newcommand{\Gr}{\mathbf{Gr}}

\newcommand{\N}{\mathbf{N}}


==> sections/._impl.tex <==
thomas@macbook.11025
